Learning to Accelerate Approximate Methods for Solving Integer Programming via Early Fixing

Integer programming (IP) is an important and challenging problem. Approximate methods have shown promising performance on both effectiveness and efficiency for solving the IP problem. However, we observed that a large fraction of variables solved by some iterative approximate methods fluctuate around their final converged discrete states in very long iterations. Inspired by this observation, we aim to accelerate these approximate methods by early fixing these fluctuated variables to their converged states while not significantly harming the solution accuracy. To this end, we propose an early fixing framework along with the approximate method. We formulate the whole early fixing process as a Markov decision process, and train it using imitation learning. A policy network will evaluate the posterior probability of each free variable concerning its discrete candidate states in each block of iterations. Specifically, we adopt the powerful multi-headed attention mechanism in the policy network. Extensive experiments on our proposed early fixing framework are conducted to three different IP applications: constrained linear programming, MRF energy minimization and sparse adversarial attack. The former one is linear IP problem, while the latter two are quadratic IP problems. We extend the problem scale from regular size to significantly large size. The extensive experiments reveal the competitiveness of our early fixing framework: the runtime speeds up significantly, while the solution quality does not degrade much, even in some cases it is available to obtain better solutions. Our proposed early fixing framework can be regarded as an acceleration extension of ADMM methods for solving integer programming. The source codes are available at \url{https://github.com/SCLBD/Accelerated-Lpbox-ADMM}.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tab3_1.tex <==
\begin{table*}[!t]
    \centering
    % \setlength{\abovecaptionskip}{0cm}
\caption{Comparative study on different methods for image segmentation on the PASCAL Visual Object Classes Challenge 2012 (VOC2012)} %, training on 12800 instances and test on 1000 instances. The method RL+LSTM is by \cite{pan2020solving}
\label{ablation}
\resizebox{17.9cm}{!}{
\begin{tabular}{lccccccccc}
    \toprule[1.5pt]
     Size \rightarrow && \multicolumn{2}{c}{$n=1\times 10^4$} & \multicolumn{2}{c}{$n=5\times 10^4$} & \multicolumn{2}{c}{$n=1\times 10^5$} & \multicolumn{2}{c}{$n=5 \times 10^5$}  \\
     \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
     Model \downarrow & Language & Energy & Runtime & Energy & Runtime & Energy & Runtime & Energy & Runtime\\
    % \midrule
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    min-cut  & M. & 12083 & 0.1s & 54409 & 0.2s & 105677 & 0.4s & 493822 & 1.8s  \\
    linear relaxation & M. & 12604 & 1.0s & 56034 & 5.5s & 108188 & 12.1s & 616240 & 121.0s     \\
    spectral relaxation & M. & 14801 & 0.1s & 67852 & 0.2s & 1398597 & 0.3s & 585554 & 1.1s   \\
    % $\ell_{1}$-box ADMM & M. & 12200 & 1.9s & 54581 & 7.2s & 105905 & 17.5s & 495638 & 99.8s  \\ 
    $\ell_{p}$-box ADMM & M. & 12200 & 1.8s & 54583 & 7.1s & 105889 & 17.8s & 495676 & 98.9s   \\
    % \midrule
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    % $\ell_{1}$-box ADMM & C.   \\
    $\ell_{p}$-box ADMM & C. & 11367 & 0.3s & 53424 & 1.3s & 106455 & 3.1s & 516213 & 19.5s  \\
    % $\ell_{1}$-box ADMM + LEF & C.+P.   \\
    $\ell_{p}$-box ADMM + LEF(MLP) & C.+P. & 11416/90 & 0.11s & 53894 & 0.55s & 107289 & 1.12s & 520199 & 5.55s  \\  
    $\ell_{p}$-box ADMM + LEF(Att.) & C.+P.& 11484/139 & 0.14s & 54083 & 0.64s & 107646 & 1.27s & 521961 & 6.67s  \\   
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    % \\
    
    Size \rightarrow && \multicolumn{2}{c}{$n=1\times10^6$} & \multicolumn{2}{c}{$n=5\times 10^6$} & \multicolumn{2}{c}{$n=1 \times 10^7$} & \multicolumn{2}{c}{$n=5\times10^7$} \\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
     Model \downarrow & Language & Energy & Runtime & Energy & Runtime & Energy & Runtime & Energy & Runtime \\
    % \midrule
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    min-cut  & M. & 954222 & 3.7s & 4418804 & 22.8s & 8587901 & 46.3s & 40942300 & 952.0s  \\
    linear relaxation & M. & 1136829 & 482.9 & 4822289 & 1152.5s       \\
    spectral relaxation & M. & 13833348 & 2.4s & 4650494 & 11.6s & 8863949 & 25.6s & 678341419 & 986.9s \\
    % $\ell_{1}$-box ADMM & M. & 957234 & 187.4s & 4440105 & 1110.8s & 8621096 &  2183.1s \\ 
    $\ell_{p}$-box ADMM & M. & 957696 & 170.3s & 4440543 & 1170.2s & 8621096 &  2183.1s & 41062236 & 91311s(25.4h) \\
    % \midrule
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    % $\ell_{1}$-box ADMM & C.   \\
    $\ell_{p}$-box ADMM & C. & 1021621 & 41.9s & 4990251 & 293.6s & 9918274 & 648.1s & 49075089 & 3143.1s   \\
    % $\ell_{1}$-box ADMM + LEF & C.+P.   \\
    $\ell_{p}$-box ADMM + LEF(MLP) & C.+P. & 1029442 & 9.98s & 5018813 & 53.5s & 9965716 & 130.89s &  49239894 & 981.1s \\ 
    $\ell_{p}$-box ADMM + LEF(Att.) & C.+P. & 1032016 & 10.79s & 5032778 & 58.9s & 9995522 & 136.18s & 49386140 & 1108.14s  \\
    \bottomrule[1.5pt]
\end{tabular}}
\end{table*}

==> tab3_2.tex <==
\begin{table*}[!t]
    \centering
    % \setlength{\abovecaptionskip}{0cm}
\caption{Comparative study on different methods for image segmentation on the PASCAL Visual Object Classes Challenge 2012 (VOC2012)} %, training on 12800 instances and test on 1000 instances. The method RL+LSTM is by \cite{pan2020solving}
\label{ablation}
\resizebox{17.9cm}{!}{
\begin{tabular}{ccccccccccc}
    \toprule[1.5pt]
     Size \rightarrow && \multicolumn{3}{c}{$n=1\times 10^5$} & \multicolumn{3}{c}{$n=5 \times 10^5$} & \multicolumn{3}{c}{$n=1\times10^6$} \\
     Model \downarrow & Language & Objective & Objective Gap & Runtime & Objective & Objective Gap & Runtime & Objective & Objective Gap & Runtime \\
    % \midrule
    \cmidrule(lr){1-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
    min-cut  & M. & 709k \pm 267k &31.0s &  31.6  \\
    linear relaxation & M. & 365k+267k &18.6s &  30.6       \\
    spectral relaxation & M. & \\
    $\ell_{1}$-box ADMM & M. \\ 
    $\ell_{2}$-box ADMM & M. \\
    % \midrule
    \cmidrule(lr){1-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
    $\ell_{1}$-box ADMM & C.   \\
    $\ell_{2}$-box ADMM & C.   \\
    $\ell_{1}$-box ADMM + LEF & C.+P.   \\
    $\ell_{2}$-box ADMM + LEF & C.+P.  \\   
    \cmidrule(lr){1-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
    \\
    
    Size \rightarrow && \multicolumn{3}{c}{$n=5\times 10^6$} & \multicolumn{3}{c}{$n=1 \times 10^7$} & \multicolumn{3}{c}{$n=5\times10^7$} \\
     Model \downarrow & Language & Objective & Objective Gap & Runtime & Objective & Objective Gap & Runtime & Objective & Objective Gap & Runtime \\
    % \midrule
    \cmidrule(lr){1-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
    min-cut  & M. & 709k \pm 267k &31.0s &  31.6  \\
    linear relaxation & M. & 365k+267k &18.6s &  30.6       \\
    spectral relaxation & M. & \\
    $\ell_{1}$-box ADMM & M. \\ 
    $\ell_{2}$-box ADMM & M. \\
    % \midrule
    \cmidrule(lr){1-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
    $\ell_{1}$-box ADMM & C.   \\
    $\ell_{2}$-box ADMM & C.   \\
    $\ell_{1}$-box ADMM + LEF & C.+P.   \\
    $\ell_{2}$-box ADMM + LEF & C.+P.  \\   
    \bottomrule[1.5pt]
\end{tabular}}
\end{table*}


\begin{table*}[!t]
    \centering
    % \setlength{\abovecaptionskip}{0cm}
\caption{Comparative study on different methods for image segmentation on the PASCAL Visual Object Classes Challenge 2012 (VOC2012)} %, training on 12800 instances and test on 1000 instances. The method RL+LSTM is by \cite{pan2020solving}
\label{ablation}
\resizebox{17.9cm}{!}{
\begin{tabular}{lccccccccc}
    \toprule[1.5pt]
     Size \rightarrow && \multicolumn{2}{c}{$n=1\times 10^4$} & \multicolumn{2}{c}{$n=5\times 10^4$} & \multicolumn{2}{c}{$n=1\times 10^5$} & \multicolumn{2}{c}{$n=5 \times 10^5$}  \\
     \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
     Model \downarrow & Language & Energy & Runtime & Energy & Runtime & Energy & Runtime & Energy & Runtime\\
    % \midrule
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    min-cut  & M. & 3300 & 0.1s & 11828 & 0.2s & 21884 & 0.4s & 84561 & 1.8s  \\
    linear relaxation & M. &  &       \\
    spectral relaxation & M. & \\
    $\ell_{1}$-box ADMM & M. &   \\ 
    $\ell_{2}$-box ADMM & M. & 3343 & 1.8s & 12113 & 7.1s & 22343 & 15.0s & 87297 & 82.9s   \\
    % \midrule
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    $\ell_{1}$-box ADMM & C.   \\
    $\ell_{2}$-box ADMM & C.   \\
    $\ell_{1}$-box ADMM + LEF & C.+P.   \\
    $\ell_{2}$-box ADMM + LEF & C.+P.  \\   
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    % \\
    
    Size \rightarrow && \multicolumn{2}{c}{$n=1\times10^6$} & \multicolumn{2}{c}{$n=5\times 10^6$} & \multicolumn{2}{c}{$n=1 \times 10^7$} & \multicolumn{2}{c}{$n=5\times10^7$} \\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
     Model \downarrow & Language & Energy & Runtime & Energy & Runtime & Energy & Runtime & Energy & Runtime \\
    % \midrule
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    min-cut  & M. & 139192 & 3.7s &   \\
    linear relaxation & M. &        \\
    spectral relaxation & M. & \\
    $\ell_{1}$-box ADMM & M. \\ 
    $\ell_{2}$-box ADMM & M. & 145260 & 170.3s \\
    % \midrule
    \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
    $\ell_{1}$-box ADMM & C.   \\
    $\ell_{2}$-box ADMM & C.   \\
    $\ell_{1}$-box ADMM + LEF & C.+P.   \\
    $\ell_{2}$-box ADMM + LEF & C.+P.  \\   
    \bottomrule[1.5pt]
\end{tabular}}
\end{table*}
